Guaranteed Model-Based Fault Detection in Cyber-Physical Systems: A Model Invalidation Approach

This paper presents a sound and complete fault detection approach for cyber-physical systems represented by hidden-mode switched affine models with time varying parametric uncertainty. The fault detection approach builds upon techniques from model invalidation. In particular, a set-membership approach is taken where the noisy input-output data is compared to the set of behaviors of a nominal model. As we show, this set-membership check can be reduced to the feasibility of a mixed-integer linear programming (MILP) problem, which can be solved efficiently by leveraging the state-of-the-art MILP solvers. In the second part of the paper, given a system model and a fault model, the concept of T-detectability is introduced. If a pair of system and fault models satisfies T-detectability property for a finite T, this allows the model invalidation algorithm to be implemented in a receding horizon manner, without compromising detection guarantees. In addition, the concept of weak-detectability is introduced which extends the proposed approach to a more expressive class of fault models that capture language constraints on the mode sequences. Finally, the efficiency of the approach is illustrated with numerical examples motivated by smart building radiant systems.

==> sec_appendices.tex <==
%!TEX root = bare_jrnl.tex

\appendix
%\setcounter{secnumdepth}{0}
\section{Appendix - Converting absolute value constraints to mixed integer linear constraints:}\label{app:abstomilp}
		Consider the first constraint in \eqref{eqn:setmilpconst}:
		\begin{equation*}
		|\mathbf{Z}^{A}_{i,k}(m,l)| \leq |\hat{\A}_{i}(m,l)||\x_{k}(l)|. 
		\end{equation*}
		This constraint is in the form of $|x|\leq C|y|, C \geq 0$ and both $x$ and $y$ are variables. Let us introduce a new variable $z=|y|$. Two cases can be considered: if $y\geq 0$, then $z=y$ and $z=-y$ vice versa. We also assign a binary variable $b$, which is 1, if $y\geq0$ and 0 otherwise. Then, $|x|\leq C|y|$ is enforced by the following linear constraints, where $M$ is an upper bound for $2|y|$:
		\begin{align*}
		-Cz \leq & x \leq Cz \\
		0 \leq & z-y \leq M (1 - b)\\
		0 \leq & z+y \leq Mb
		\end{align*}
		
%		Next, we show how we can replace such a constraint with linear constraints.
%		If $|[\A^{N}_{i}]^{m,l}|$ is zero, then $\pmb{\delta}^{A^{m_l}}_{i,k}=0$ and both the new variable and constraint can be removed. Otherwise, it is a positive constant, and we can divide both sides of inequality by that and define new variables as follows:
%		\begin{equation*}
%		|\pmb{\sigma}^{A^{m_l}}_{i,k}| \leq |\z'^l_{i,k}|
%		\end{equation*}
%		There are four different cases that are possible, and if any of them occurs, then the constraint above is satisfied. 
%		In fact only one of the following four cases can occur at each time, so the constraint above is equivalent to the 
%		logical OR of the following four cases: 
%			
%		\begin{itemize}
%			\item $\pmb{\sigma}^{A^{m_l}}_{i,k}\geq 0, \z'^l_{i,k} \geq 0, \pmb{\sigma}^{A^{m_l}}_{i,k} \leq \z'^l_{i,k}$
%			\item $\pmb{\sigma}^{A^{m_l}}_{i,k}\leq0, \z'^l_{i,k}\leq0, \pmb{\sigma}^{A^{m_l}}_{i,k} \geq \z'^l_{i,k}$
%			\item $ \pmb{\sigma}^{A^{m_l}}_{i,k}\geq 0, \z'^l_{i,k} \leq 0, \pmb{\sigma}^{A^{m_l}}_{i,k} \leq -\z'^l_{i,k}$
%			\item $ \pmb{\sigma}^{A^{m_l}}_{i,k} \leq 0, \z'^l_{i,k} \geq 0, \pmb{\sigma}^{A^{m_l}}_{i,k} \geq -\z'^l_{i,k}$
%		\end{itemize}
%		In order to implement the logical OR between the four cases, we need to introduce four binary variables: 
%		$b_1,b_2,b_3,b_4$. The equivalent MIP constraints are as follows:
%		\begin{align}
%			& b_1\pmb{\sigma}^{A^{m_l}}_{i,k} \geq 0, \; b_1\z'^l_{i,k} \geq 0,\; b_1(\pmb{\sigma}^{A^{m_l}}_{i,k}-\z'^l_{i,k}) \leq 0 \\
%			& b_2\pmb{\sigma}^{A^{m_l}}_{i,k} \leq 0,\; b_2\z'^l_{i,k} \leq 0,\; b_2(\pmb{\sigma}^{A^{m_l}}_{i,k}-\z'^l_{i,k}) \geq 0 \\
%			& b_3\pmb{\sigma}^{A^{m_l}}_{i,k} \geq 0,\; b_3\z'^l_{i,k} \leq 0,\; b_3(\pmb{\sigma}^{A^{m_l}}_{i,k}+\z'^l_{i,k}) \leq 0 \\
%			& b_4\pmb{\sigma}^{A^{m_l}}_{i,k} \leq 0,\; b_4\z'^l_{i,k} \geq 0,\; b_4(\pmb{\sigma}^{A^{m_l}}_{i,k}+\z'^l_{i,k}) \geq 0 
%		\end{align}
%		with  $\textstyle \sum_{i\in \mathbb{Z}^+_4} b_i = 1$.
%			Finally, in order to transform these constraints to MILP, we define $\tilde{\z}^l_{i,q,k} \doteq b_q \z'^l_{i,k}$, 
%			$\pmb{\sigma}^{A^{m_l}}_{i,q,k} \doteq b_q\pmb{\sigma}^{A^{m_l}}_{i,k}$ and $\tilde{a}_{i,q,k}\doteq a_{i,k}b_q$. Therefore, $\textstyle \sum_{q\in \mathbb{Z}^+_4}\tilde{\z}^l_{i,q,k} = \z'^l_{i,k}$ and $\textstyle \sum_{q\in \mathbb{Z}^+_4} \tilde{a}_{i,q,k} = a_{i,k}$. The following constraints ensure that $ \pmb{\sigma}^{A^{m_l}}_{i,q,k}, \tilde{\z}^l_{i,q,k}$ are only nonzero for one of the four cases, without adding any extra constraints. 
%			\begin{align*}
%			\tilde{a}_{i,q,k}X_l  \leq & \pmb{\sigma}^{A^{m_l}}_{i,q,k} \leq \tilde{a}_{i,q,k}X_u \\
%			\tilde{a}_{i,q,k} X_l \leq & \tilde{\z}^l_{i,q,k} \leq \tilde{a}_{i,q,k}X_u.
%			\end{align*}
			
			
			%	\section{Proof of Proposition \ref{pro:mimilp}} \label{app:prop1proof}
			%		We denote $\x_k, \; \ETA_k, \; \A^\Delta_{i,k},\; \B^\Delta_{i,k}, \; \C^\Delta_{i,k}, \; \f^\Delta_{i,k}, \; a_{i,k}$ as
			%		 \eqref{eqn:feasoptnonlineartot} variables and $\z_{i,k},\z'_{i,k}, \THE_{i,k}, \Delta^{A,x}_{i,k}, \Delta^B_{i,k}, 
			%		 \Delta^{C,x}_{i,k}, a_{i,k}$ as \eqref{eqn:uncmilp} variables. The change of variables in Table 2 are defined as
			%		  the transform from \eqref{eqn:feasoptnonlinear1} variables to \eqref{eqn:uncmilp} variables. The proof has two parts:
			%		\subsection{Sufficient condition}
			%		We show that a general feasible point of \eqref{eqn:feasoptnonlinear1} maps to a feasible point of \eqref{eqn:uncmilp}.
			%		
			%		Assumption: $\x_k, \; \ETA_k, \; \A^\Delta_{i,k},\; \B^\Delta_{i,k}, \; \C^\Delta_{i,k}, \; \f^\Delta_{i,k}, \; a_{i,k}$
			%		 is a feasible point of \eqref{eqn:feasoptnonlinear1} for $\forall k \in \mathbb{Z}_{N-1}^0, \forall i\in \mathbb{Z}_s^+$. 
			%		
			%		We pursue by claiming that if we choose \eqref{eqn:uncmilp} variables to be Table 1 transformation 
			%		of \eqref{eqn:feasoptnonlinear1} feasible point, then this choice is a feasible point of \eqref{eqn:uncmilp}. 
			%		This is shown by verifying that these transformed variables satisfy every constraint in \eqref{eqn:uncmilp}. 
			%		For all the constraints, we begin with a constraint in \eqref{eqn:uncmilp} and replace the variables with 
			%		\eqref{eqn:feasoptnonlinear1} variables, and show that it results in a feasible constraint for \eqref{eqn:feasoptnonlinear1}, 
			%		therefore it is feasible for \eqref{eqn:uncmilp}. 
			%		
			%		Constraint \eqref{eqn:ORmilpconst1}: By replacing \eqref{eqn:uncmilp} variables with the ones of 
			%		\eqref{eqn:feasoptnonlinear1} we have:
			%		\begin{equation*}
			%		\begin{aligned}
			%		a_{i,k}\x_{k+1} = & a_{i,k}(\mathbf{A}_{i}+\A^\Delta_{i,k}) \x_k +  a_{i,k}(\B_{i}+\B^\Delta_{i,k})   \mathbf{u}_k+  \\ 
			%		& a_{i,k}\mathbf{f}_{i} + a_{i,k}\f^\Delta_{i,k},
			%		\end{aligned}
			%	\end{equation*}
			%		which is feasible from the feasibility of \eqref{eqn:feasoptnonlinear1}.
			%		
			%		Constraint \eqref{eqn:ORmilpconst2}: The same approach gives us:
			%		\begin{equation*}
			%		a_{i,k}\mathbf{y}_k = a_{i,k}(\C_{i}+\C^\Delta_{i,k})  \x_k +a_{i,k}\ETA_k,
			%		\end{equation*}
			%		which again is feasible.
			%		
			%		Constraint \eqref{eqn:ORmilpconst3}: is a common constraint between the two problem, hence choosing the 
			%		same $a_{i,k}$ variables makes \eqref{eqn:ORmilpconst3} feasible as well.
			%		
			%		Constraint \eqref{eqn:ORmilpconst4}: Replacement of variables results in:
			%		\begin{align*}
			%		& \sum_{i=1}^{s} a_{i,k}x_{k+1} = \sum_{i=1}^{s} a_{i,k+1}x_{k+1} \implies \\ & x_{k+1}\sum_{i=1}^{s} a_{i,k} = 
			%		x_{k+1}\sum_{i=1}^{s} a_{i,k+1} \implies x_{k+1} = x_{k+1},   
			%		\end{align*} 
			%		which is feasible. The last equality is obtained because $\sum_{i=1}^{s} a_{i,k} = \sum_{i=1}^{s} a_{i,k+1} = 1$.
			%		
			%		Constraint \eqref{eqn:setmilpconst1}: By replacing the variables we have:
			%		\begin{equation*}
			%		a_{i,k} T_l \leq a_{i,k} t_k \leq a_{i,k} T_u.  
			%	\end{equation*}
			%		The equation above is feasible for $T_l \leq t_k \leq T_u$, where $(t,T)$ are either $(\x, X)$ or $(\ETA, \epsilon )$.
			%		
			%		Constraint \eqref{eqn:setmilpconst2}: Using the transformation of variables we have:
			%	\begin{equation*}	
			%		-a_{i,k} \leq a_{i,k} Q^{\Delta}_{i,k} \leq a_{i,k},
			%	\end{equation*}
			%		clearly this is feasible for $-1 \leq Q^{\Delta}_{i,k} \leq 1$, where $Q \in \{\B, \f \}$.
			%		
			%		Constraint \eqref{eqn:setmilpconst3}: By transforming the variables we have:
			%		\begin{equation*} 
			%		\begin{aligned}
			%		& |\Delta T^{m,l}_{i,k} \z'^l_{i,k} | \leq |\z'^l_{i,k}| \\
			%		& \text{ if } \z'^l_{i,k} = 0, \text{ we have }0 \leq 0, \text{which is feasible} \\ 
			%		& \text{Otherwise divide both sides by $|\z'^l_{i,k}|$} \implies |{\Delta}_{T,i,k}| \leq 1,
			%		\end{aligned}
			%	\end{equation*}
			%		which is feasible for $T \in \{ \A, \C \}$. Here, $m,l$ can be any value from 1 to the number of rows and columns of 
			%		$T$, respectively.
			%		
			%		This concludes that the feasibility of \eqref{eqn:feasoptnonlinear1} implies the feasibility of \eqref{eqn:uncmilp}.
			%		\subsection{Necessary condition} 
			%		In the second part of proof, we aim to show that a feasible point of \eqref{eqn:uncmilp} maps indeed to a feasible 
			%		point of \eqref{eqn:feasoptnonlinear1}. This time we start with the constraints in \eqref{eqn:feasoptnonlinear1} and 
			%		show that they are feasible if we choose \eqref{eqn:feasoptnonlinear1} variables to be the inverse mapping of Table 
			%		\ref{tab:changeofvmi} on a feasible point of \eqref{eqn:uncmilp}.
			%		
			%		Constraint \eqref{eqn:stateconst0}: By replacing \eqref{eqn:feasoptnonlinear1} variables with \eqref{eqn:uncmilp} variables,
			%		 we obtain \eqref{eqn:ORmilpconst1}, which is feasible due to the feasibility of \eqref{eqn:uncmilp}.
			%		
			%		Constraint \eqref{eqn:stateconst1}: With similar strategy, we obtain \eqref{eqn:ORmilpconst2}, which is also feasible.
			%		
			%		Constraint \eqref{eqn:stateconstbin}: This is a common constraint, hence feasible.
			%		
			%		Constraint \eqref{eqn:stateconst2}: We know that at each time instance $k$ there is a mode $i^*$, where $a_{i^*,k} = 1$. 
			%		Consider $\z'_{i^*,k}$, from feasibility of \eqref{eqn:uncmilp}, we know that:
			%		\begin{equation*}
			%		a_{i^*,k} T_l \leq a_{i^*,k} t_k \leq a_{i^*,k} T_u, \;  a_{i^*,k}=1
			%	\end{equation*} 
			%		is feasible for $(t,T)$ being either $ (\x, X)$ or $(\ETA, \epsilon)$. Hence, \eqref{eqn:stateconst2} is feasible.
			%		
			%		Constraint \eqref{eqn:stateconst3}: From feasibility of \eqref{eqn:setmilpconst2} with the same argument as above, 
			%		the feasibility of \eqref{eqn:stateconst3} is verified for $T \in \{ \B, \f \}$. For $T \in \{\A, \C \}$ we have:
			%		\begin{equation*}
			%		-1\leq \Delta^{m,l}_{T,i,k} \leq 1, T\in \{ \A,\C\} \implies  | \Delta^{m,l}_{T,i,k}| \leq 1
			%	\end{equation*}
			%		is feasible. if we multiply this inequality with a positive number, we don't change the feasibility. We multiply both sides 
			%		with $|\z'^l_{i^*,k}|$. Then we have:
			%		\begin{equation*}
			%		| \Delta^{m,l}_{T,i,k} \z'^l_{i^*,k}| \leq |\z'^l_{i^*,k}|
			%	    \end{equation*}
			%		which is feasible from the feasibility of \eqref{eqn:uncmilp}. Therefore, \eqref{eqn:stateconst3} is feasible.
			%		
			%		This completes the second part, which means feasibility of \eqref{eqn:uncmilp} implies the feasibility of 
			%		\eqref{eqn:feasoptnonlinear1}. This concludes the proof, as we showed \eqref{eqn:feasoptnonlinear1} is 
			%		feasible if and only if \eqref{eqn:uncmilp} is feasible.
			%		
		 
%\end{appendices}
